Poncelet Propellers: Invariant Total Blade Area

Given a triangle, a trio of circumellipses can be defined, each centered on an excenter. Over the family of Poncelet 3-periodics (triangles) in a concentric ellipse pair (axis-aligned or not), the trio resembles a rotating propeller, where each "blade" has variable area. Amazingly, their total area is invariant, even when the ellipse pair is not axis-aligned. We also prove a closely-related invariant involving the sum of blade-to-excircle area ratios.

==> 999_latex_examples.tex <==
exemples:

I showed before that $a=b+c$ and $a_2=b_2+c_2$. However:

\[ a = b + c \] % une seule equation

Therefore:

\begin{equation*}
    a_2 = b_2 + c_2 % ne prendra pas de nombre
\end{equation*}

\begin{equation}
    a = b + c % prendra un nombre style (1)
    \label{eqn:mon-eqn}
\end{equation}

On a vu sur \eqref{eqn:mon-eqn} que ...


\begin{align*}
    a & = b + c \\
    d & = e + f + g \\
    h & = a + b + f \\
      & + z_1 + z_2
\end{align*}

\begin{align}
    a =\, & b + c \nonumber \\
    d =\, & e + f + g \label{eqn:ddd} \\
    h =\, & a + b + f +g + j + k + \nonumber\\
      & z_1 + z_2 \nonumber
\end{align}

In \eqref{eqn:ddd} we talked about...

==> app_120_triangle_geometry.tex <==

%\textcolor{red}{dominique i don't understand}
%\textcolor{green}{dan, is it better with subsection titles ?}

%\subsection{Trilinear coordinates definition}

%The so-called ``exact trilinear coordinates'' $u,v,w$ of a triangle $P_1 P_2 P_3$ are shown in Figure~\ref{fig:exact-trilinears}.

%\begin{figure}
%    \centering
%    \includegraphics[width=.7\textwidth]{pics/pics_120_trilinear_coordinates.eps}
%    \caption{Exact trilinear coordinates $u,v,w$ for triangle $P_1 P_2 P_3$ with side lengths $s_1,s_2,s_3$.}
    \label{fig:exact-trilinears}
%\end{figure}



%\subsection{Inellipse area formula}

%Squared area of an $P_1 P_2 P_3$ inellipse ${\mathcal{E}_1}$ is
%
%\begin{align*}
%    \Delta_{\mathcal{E}_1}^2 = \pi^2 ( 1 - 2 m_1 ) ( 1 - 2 m_2 ) ( 1 - 2 m_3 ) S^2
%\end{align*}
%
%where $m_1 : m_2 : m_3$ are the homogeneous barycentric coordinates of Brianchon point O with respect to $P_1, P_2,P_3$ and S is $P_1 P_2 P_3$ area.
